Contamination of Dark Matter Experiments from Atmospheric Magnetic Dipoles

Dark matter collisions with heavy nuclei (Xe, Ge, Si, Na) may produce recoils observable at direct-search experiments. Given that some of these experiments are yielding conflicting information, however, it is worth asking if physics other than dark matter may produce similar nuclear recoils. We examine under what conditions an atmospherically-produced neutral particle with a relatively large magnetic dipole moment could fake a dark matter signal. We argue that a very definite flux could explain the signals seen at DAMA/LIBRA, CDMS/Si and CoGeNT consistently with the bounds from XENON100 and CDMS/Ge. To explore the plausibility of this scenario, we discuss a concrete model with 10-50 MeV sterile neutrinos that was recently proposed to explain the LSND and MiniBooNE anomalies.

==> cmds/format-science-supersymmetry.tex <==
% <!DOCTYPE LaTeX2e>
%
% <info>
% 	supersymmetry formatting commands
% </info>
%
%	Superfields (both vector and chiral)
	\newcommand{\superf}[1]{\mathcal{#1}}
%	Superfield Strength
	\newcommand{\superstrn}[1]{\mathscr{#1}}
%	super derivative
	\newcommand{\superD}{\mathpzc{D}}
	\newcommand{\superDbar}{\overline{\mathpzc{D}}}
%	Vector Superfield fermion
	\newcommand{\gaugino}[1]{\mathrm{\MakeLowercase{#1}}}
%	Scalar Component of superfield
	\newboolean{ulinescalar}
	\newcommand{\scalarunderline}{\setboolean{ulinescalar}{true}}%
	\newcommand{\noscalarunderline}{\setboolean{ulinescalar}{false}}%
	\newcommand{\scalar}[1]{%
		\ifthenelse{ \boolean{ulinescalar} }
			{
			\ifx#1\DeltaC%
				{%
				\underline{\Delta}^c%
				% \delta^c
				}%
			\else\ifx#1\DeltaBarC%
				{%
				\underline{\bar{\Delta}}^c%
				% \bar{\delta}^c
				}%
			\else\ifx#1\Phi%
				{%
				\underline{\Phi}%
				% \phi
				}%
			\else\ifthenelse{ \equal{#1}{L^c}}%
				{%
				\underline{L}^c%
				% \ell^c
				}%
			{\ifthenelse{ \equal{#1}{Q^c}}%
				{%
				\underline{Q}^c%
				% q^c
				}%
			{\ifthenelse{ \equal{#1}{H_u}}%
				{%
				\underline{H}_u%
				% h_u
				}%
			{\ifthenelse{ \equal{#1}{H_d}}%
				{%
				\underline{H}_d%
				% h_d
				}%
			% Else
				{%
				\underline{#1}%
				% \expandafter\MakeLowercase{#1}
				}}}}%
			\fi\fi\fi
			}
		% Else
			{
			#1%
			}
		}%

==> cmds/preamble-cmd-spectrum_draw.tex <==
\let\gobbleEnd=\relax
\newcommand{\drawmasslines}[2]{\gobblemasslist#2,\gobbleHalt\gobbleEnd}
\newcommand{\gobbleHalt}{\@\@\@\@}

\def\gobblemasslist(#1,#2,[#3,#4]),#5\gobbleEnd{%
\ifthenelse{ \equal{#5}{\gobbleHalt} }%
	{%
	\put(\xCoord,#2){\line(1,0){\masslinelen} \raisebox{#4}{\hspace{#3}$#1$}}%
	}%
% Else
	{%
	\put(\xCoord,#2){\line(1,0){\masslinelen} \raisebox{#4}{\hspace{#3}$#1$}}%
	\gobblemasslist#5\gobbleEnd%
	}%
}%


\newlength{\oldunitlength}
\setlength{\oldunitlength}{\the\unitlength}
\newcommand{\masslinelen}{50}
\newcommand{\xCoordColOne}{10}
\newcommand{\xCoordColTwo}{120}
\newcommand{\xCoordColThree}{230}
\newcommand{\xCoordColFour}{340}
\newcommand{\xCoordColFive}{450}
\newcommand{\xCoord}{}
\newcommand{\defaultX}{1mm}
\newcommand{\defaultY}{-0.6ex}
\newcommand{\placetoleft}{-1.4cm}
\newcommand{\placetoleftnudgeright}{-1.33cm}
\newcommand{\placetoleftnudgeleft}{-1.47cm}
\newcommand{\slightlyraised}{-0.4ex}
\newcommand{\slightlylowered}{-0.8ex}


